NPF-200: A Multi-Modal Eye Fixation Dataset and Method for Non-Photorealistic Videos

Non-photorealistic videos are in demand with the wave of the metaverse, but lack of sufficient research studies. This work aims to take a step forward to understand how humans perceive non-photorealistic videos with eye fixation (\ie, saliency detection), which is critical for enhancing media production, artistic design, and game user experience. To fill in the gap of missing a suitable dataset for this research line, we present NPF-200, the first large-scale multi-modal dataset of purely non-photorealistic videos with eye fixations. Our dataset has three characteristics: 1) it contains soundtracks that are essential according to vision and psychological studies; 2) it includes diverse semantic content and videos are of high-quality; 3) it has rich motions across and within videos. We conduct a series of analyses to gain deeper insights into this task and compare several state-of-the-art methods to explore the gap between natural images and non-photorealistic data. Additionally, as the human attention system tends to extract visual and audio features with different frequencies, we propose a universal frequency-aware multi-modal non-photorealistic saliency detection model called NPSNet, demonstrating the state-of-the-art performance of our task. The results uncover strengths and weaknesses of multi-modal network design and multi-domain training, opening up promising directions for future works. {Our dataset and code can be found at \url{https://github.com/Yangziyu/NPF200}}.

==> section4-method-bk.tex <==


\section{Method}\label{method}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{figure/saliency_network.pdf}
	\vspace*{-1.8mm}
	\caption{The pipeline of our NPSNet. Given the current frame from a non-photorealistic video with its visual context ($k-1$ preceding frames) and corresponding audio waveform of these $k$ frames, our model can predict the saliency map of current frame. }
	\label{fig:method}
\end{figure*}



We propose \textbf{NPSNet} (Non-Photorealistic Saliency Network) that aims to achieve saliency detection for non-photorealistic video with audio. Instead of sending only a single frame $I_i$ into the network to predict the saliency map $M_i$, for the $n-th$ frame, we also input its multi-modal context, 1) visual context with $k-1$ frames before the current frame, and 2) audio context with the corresponded soundtrack of these $k$ frames. Since the viewer's attention is often followed with continuous action and scene changes of the video, our inputs allow the model to better capture such temporal and auxiliary information.


%As shown in \reffig{method}, our model consists of Multi-Modal Feature Extraction, Video-Audio Interaction and Saliency Prediction.
%In this section, we first clarify the definition of saliency prediction, then we introduce the function and composition
%of each module of NPSNet. Finally, we illustrate the training and testing process of NPSNet.

%\subsection{Problem Definition}
%We consider the general setting of saliency prediction. The definition of saliency prediction is formulated as follow: given
%a $K$-frames video clip $\boldsymbol{V}=\left\{I_{(1)}, \ldots, I_{(K)}\right\}$ and its corresponding $K$ saliency
%maps $\boldsymbol{M}=\left\{M_{(1)}, \ldots, M_{(K)}\right\}$, the goal of saliency prediction network is to predict saliency map
%$S_{(n)}(\text {n} \in[1, \ldots, K])$ of each video frame $I_{(n)}(\text {n} \in[1, \ldots, K])$ under the supervision of $M_{(n)}(\text {n} \in[1, \ldots, K])$.
%However, the form of inputting a frame and outputting a saliency map is unreliable.\todo{unclear} The first reason is that a continuous sequence of video frames can provide temporal and spatial information to our network.
%The second reason is that for frames 1 to $t(\text {t}\le K)$, when the value of $t$ is not large, adjacent video frames have continuous action and scene changes, and people's visual attention is roughly followed.
%The difference of saliency maps between adjacent video frames is small. Both of these factors favor the network learning to predict saliency maps from continuous video sequences.
%So in our method, we set a sliding window of size $t$ to slide the video frames, and the network only predicts the last frame of the window each time. see \refsec{train_test} for details.
%%However, when the value of k is not large, the adjacent video frames have slight object movement and action changes,
%%and therefore the difference in the saliency map of adjacent video frames is small.
%%So in our method, only the saliency map $S_{(K)}$ of the last frame $I_{(K)}$ in the video clip $I_{(n)}(\text {n} \in[1, \ldots, K])$ is predicted during training.
%%Still, the saliency map of each frame can be predicted at test time, see \refsec{train_test} for details.


\subsection{Multi-Modal Feature Extraction}
To extract the temporal and spatial features of the input video clip, we introduce a multi-modal feature extraction module composed of VideoNet with video frames as the input and AudioNet with the audio waveform as the input.

%This module is mainly composed of VideoNet and AudioNet, and its function is to extract the temporal and spatial information of the input video frame and extract the audio representation of the input audio waveform.

\textbf{AudioNet.}
We adopt seven layers SoundNet\cite{aytar2016soundnet} as the architecture of our AudioNet. Benefiting from transfer learning, this model is pretrained on audio-visual scene classification task to learn to better extract audio representation. The audio waveform first be preprocessed by a Hanning window for providing higher weight to the interested time instance before feeding into the AudioNet to obtain the audio features.
%To obtain audio representation, we refer to the audio pre-processing method of \cite{tsiami2020stavis}. Specifically, the audio waveform corresponding to the input video frames is cropped from the whole audio waveform,
%and the central audio value representing the current temporal instance is weighted using a Hanning window. The pre-processed audio waveform is fed into AudioNet to obtain an audio feature map representing the input audio information. 
%and followed by a 1$\times$1 convolution and flatten operation to obtain a fixed-length audio vector representing the input audio information.

\textbf{VideoNet.}
To efficiently extract the temporal and spatial visual feature of video, we select video swin transformer\cite{liu2022video} model as the architecture of our VideoNet. It accepts three-dimensional video frame input including the time dimension, and uses swin transformer block and patch merging to simulate the convolutional neural network to continuously reduce token proficiency and increase the receptive field of each token to reduce the amount of calculation and improve performance. In order to provide VideoNet with temporal and spatial prior knowledge of video, we load the video swin transformer parameters pretrained on Kinetics dataset\cite{kay2017kinetics} for action recognition into VideoNet.
We extract the visual feature maps by sending the video frames into VideoNet.
Meanwhile, we also extract feature maps from the shallow and deep layers of VideoNet, which contain low-level structural features and high-level semantic features, respectively.
These features are used for long-range skip concatenation to aid saliency map detection.
%To efficiently extract the temporal and spatial visual feature of video, we select S3D\cite{xie2018rethinking} model as the architecture of our VideoNet. It utilizes spatial and temporal separable 3D convolution instead of standard 3D convolution
%to achieve efficient computing performance and high recognition accuracy on on video classification. In order to provide VideoNet with temporal and spatial prior knowledge of video, we load the S3D parameters pretrained on Kinetics dataset\cite{kay2017kinetics} for action recognition into VideoNet.
%We extract the visual feature maps by sending the video frames into VideoNet.
%%%After the input video frames are fed into VideoNet, we get video feature map that contains both temporal and spatial information. 
%Meanwhile, we also extract feature maps from the shallow and deep layers of VideoNet, which contain low-level structural features and high-level semantic features, respectively.
%These features are used for long-range skip concatenation to aid saliency map detection.

%Besides, this module includes a modality gate and a flatten operation. The former can control whether NPSNet has audio input(see \refsec{train_test} for more details), and the latter can convert the feature maps of audio and video into feature vectors. \todo{highlight this?}

\rsc{
\textbf{Universal Frequency-aware Module.}} The human visual system has been observed to extract visual elementary features at varying frequencies~\cite{bullier2001integrated}. Low frequencies tend to provide global information about a given visual stimulus, such as objects of considerable size that consistently appear throughout a video, as well as accompanying audio. Conversely, high frequencies convey local spatial changes in the visual stimulus, typically related to objects of smaller sizes and with vast temporal variance in videos, and also informative audio clips with short durations. These observations suggest that the human visual system processes visual information in a frequency-dependent manner, with different frequencies carrying distinct information about the visual stimulus. To accurately and comprehensively model these features in both audio and video formats, we propose the Universal Frequency-aware Module, which is capable of capturing both high- and low-frequency information. The proposed module consists of specially designed high-frequency filters that are capable of capturing information across short ranges, such as small salient objects or objects that undergo rapid and drastic variations in a short time span:
\begin{equation}
    \begin{split}
        \hat{X}_i &= FC({X}_i; \theta), \\
        X_i^h &= Conv(\hat{X}_i; \theta)
    \end{split}
\end{equation}
where $FC(\star; \theta)$ is fully connected layer and $Conv(\star; \theta)$ is depth-wise convolution.

The low-frequency filters are in parallel with high-frequency filters to capture the information across long ranges in the feature map like large salient objects and segments of audio with long lengths that contain significant information:
\begin{equation}
    X_i^l = MSA(X_i)
\end{equation}
where $MSA(\star)$ is the multi-head self-attention.

The above filters are for spatial information, we design the third branch for channel information filtering:
\begin{equation}
    \begin{split}
        e_i = FC(Pool(X_i);\theta), \\
        X_i^c = e_i\odot X_i
    \end{split}
\end{equation}
where $Pool(\star)$ is the pooling operation. By incorporating such advanced techniques into our models, we aim to establish a universally effective approach to the analysis of eye fixation in both audio and video formats. This would contribute significantly to the development of more sophisticated and robust models for analyzing visual attention and perceptual processing. This module is placed in the video and audio net to enhance the extraction of multi-frequency features.


\subsection{Visual-Audio Interaction} 
In the previous module, we explored how to obtain temporal and spatial visual features and corresponding audio features. However, there is an essential gap between of video and audio modality.
The goal of this module is to fuse video and audio modality with the inter-modal correspondence and intra-modal correspondence.

\textbf{Inter-modal correspondence.}
Audio features and visual features extracted from a video clip belong to two modalities, but they have implicitly associated semantic information. Specifically, the audio must be aligned with the video frames in order to achieve audio-video synchronization.
For example, in games and cartoon, the video frames of the characters moving should correspond to the audio of footsteps; in the shooting game, the shooting should have corresponded visual and sound effect during combat.
Therefore, we need to explore how to bridge the gap and construct the correspondence between these two modalities, that is, to locate the position of the audio in the video frames.
To connect these two modalities, we utilize bilinear transformation to construct the inter-modal correspondence of the audio features and visual features. 
Concretely, given the audio feature vector $h_{a} \in \mathbb{R}^{k \times d_{a}}$ and video feature vector $h_{v} \in \mathbb{R}^{k \times d_{v}}$, we calculate inter-modal correspondence through bilinear transformation as follows:

\begin{equation}
    \begin{aligned}
        A=h_{a}^{T}W h_{v}+b
    \text{,}
    \end{aligned}
  \end{equation}
  where $W \in \mathbb{R}^{d_{a} \times d_{o} \times d_{v}}$ and $b \in \mathbb{R}^{d_{o} \times 1} $ are learning parameters, $d_a, d_v, d_o$ are the dimensions of $h_a, h_v, A$, respectively. And we obtain the video-audio affinity vector $A \in \mathbb{R}^{k \times d_{o}}$, which indicates inter-modal relation. 

\textbf{Intra-modal correspondence.}
Except exploring the inter-modal correspondence, the intra-modal correspondence shares the same importance. Given the continuity nature of audiences' attention on consecutive frames, we use the self-attention mechanism to help model such a case. 
%After inter-modal interaction and fusion, we hope to explore the intra-modal correspondence of video-audio affinity vector. Because the self-attention mechanism is a method capable of exploring the internal structure of the data, we choose a self-attention encoder to explore intra-modal correspondence. \todo{motivation is not well elaborated}
%In particular, since people's attention in the saliency map is not concentrated in a small area, and the saliency prediction of temporally adjacent frames are similar, long-range dependencies and temporal relationships are particularly important in saliency prediction.
We select the VIT\cite{dosovitskiy2020image} encoder, which is good at resolving long-range dependencies and temporal relations, as the architecture of our self-attention encoder.
And we load VIT parameters pretrained on the kinetics dataset\cite{kay2017kinetics} to provide video temporal and spatial priors.
Specifically, since the transformer architecture is permutation-invariant\cite{carion2020end}, we add the video-audio affinity vector and a fixed positional encoding to the self-attention encoder.
The output of our self-attention encoder goes through a 3D convolution and a 3D adaptive average pooling to obtain the saliency feature map. 
%\todo{considering to also write equations to elaborate this}

\subsection{Saliency detection}
The saliency decoder adopts six 3D convolutional layers combined with trilinear upsampling to map the saliency features to the output saliency map. Besides, the object position of the input video frames
and the output saliency map are spatially correlated, and the structural features and semantic features we extracted from the shallow and deep layers of VideoNet contain the information of the object position.
So we concatenate these  feature maps into the output of each layer in the middle of the saliency decoder and then input it to the next layer. Finally we obtain the saliency map, which indicates the area of people's visual attention of the input interested frame.

\subsection{Loss Function}\label{sec:train_test}
%\textbf{Loss Function.}
%We train our model with the supervision signal provided by the saliency maps from NPF-200 dataset. To guide NPSNet to predict reasonable saliency maps, we utilize KLD (kullback-leibler divergence) as the training loss function, which is a measure of the difference between the two probability distributions $P$ and $Q$ and widely used for saliency model. The KLD loss function can be defined as follows:
%
%\begin{equation}
%  \begin{aligned}
%    \mathcal{L}_{KLD}(P, Q)=\sum_{i} Q_{i} \log \left(\epsilon+\frac{Q_{i}}{P_{i}+\epsilon}\right)
%  \text{,}
%  \end{aligned}
%\end{equation}
%where $P$ and $Q$ are output saliency map and Ground-Truth respectively, and $\epsilon$ is a small number for regularization. 
%%\todo{change this loss to related to our task rather than a general loss any work can be used :). Give a symbol to our gt and output with their distributions, then define the corresponding loss function.}

We train our model with the supervision signal provided by the saliency maps from NPF-200 dataset. 
To guide NPSNet to predict reasonable saliency maps, we use KLD (kullback-leibler divergence) 
as the training loss function to measure the difference between the two probability distributions 
$P$ (predicted saliency map $P \in [0,1]^{h,w}$) and $Q$ (ground truth saliency map $Q \in [0,1]^{h,w}$). 
The KLD loss function can be defined as follows:
\begin{equation}
  \begin{aligned}
    \mathcal{L}_{KLD}(W|P,Q)=\sum_{x,y}Q(x,y;W)log \left(\epsilon + \frac{Q(x,y;W)}{P(x,y;W)+\epsilon}\right) 
\text{,}
  \end{aligned}
\end{equation}
where $W$ is the training parameters, and $\epsilon$ is a small number for regularization. 

\begin{comment}
\subsection{Loss Function}\label{sec:train_test}
%\textbf{Loss Function.}
We train our model with the supervision signal provided by the saliency maps from NPF-200 dataset. To guide NPSNet to predict reasonable saliency maps, we utilize KLD (kullback-leibler divergence) as the training loss function, which is a measure of the difference between the two probability distributions $P$ and $Q$ and widely used for saliency model. The KLD loss function can be defined as follows:


\begin{equation}
  \begin{aligned}
    \mathcal{L}_{KLD}(P, Q)=\sum_{i} Q_{i} \log \left(\epsilon+\frac{Q_{i}}{P_{i}+\epsilon}\right)
  \text{,}
  \end{aligned}
\end{equation}
where $P$ and $Q$ are output saliency map and Ground-Truth respectively, and $\epsilon$ is a small number for regularization.
%\todo{change this loss to related to our task rather than a general loss any work can be used :). Give a symbol to our gt and output with their distributions, then define the corresponding loss function.}

%\textbf{Inference.}
%We set a sliding window of $t=32$ frames (about 1 second) to read the training and testing video sequences. The network only predicts the saliency map of the last frame in the sliding window at a time.
%For the window of the first 32 frames, we repeat the first frame to fill the window.
%Note that our method does not require training two models to handle the case with and without audio separately. The modality gate can easily replace the input audio with a zero vector instead of retraining the model.
\end{comment}

